Late-Onset Circumstellar Medium Interactions are Rare: An Unbiased GALEX View of Type Ia Supernovae

Using ultraviolet (UV) light curves we constrain the circumstellar environments of 1080 Type Ia supernovae (SNe Ia) within $z<0.5$ from archival Galaxy Evolution Explorer (GALEX) observations. All SNe Ia are required to have pre- and post-explosion GALEX observations to ensure adequate subtraction of the host-galaxy flux. Using the late-time GALEX observations we look for the UV excess expected from any interaction between the SN ejecta and circumstellar material (CSM). Four SNe Ia are detected near maximum light and we compare the GALEX photometry to archival data, but we find none of our targets show convincing evidence of CSM interaction. A recent Hubble Space Telescope (HST) survey estimates that $\sim6\%$ of SNe Ia may interact with distant CSM, but statistical inferences are complicated by the small sample size and selection effects. By injecting model light curves into our data and then recovering them, we constrain a broad range of CSM interactions based on the CSM interaction start time and the maximum luminosity. Combining our GALEX non-detections with the HST results, we constrain occurrence of late-onset CSM interaction among SNe Ia with moderate CSM interaction, similar to that observed in PTF11kx, to $f_\text{CSM}\lesssim5.1\%$ between $0-500$ days after discovery and $\lesssim2.7\%$ between $500-1000$ days after discovery at $90\%$ confidence. For weaker CSM interactions similar to SN 2015cp, we obtain limits of $\lesssim16\%$ and $\lesssim4.8\%$, respectively, for the same time ranges.

==> 2021 SNe Ia-CSM in GALEX 2021-11-18/constraints.tex <==
\begin{deluxetable*}{LLDDDLL}
\tablecaption{\normalsize Upper 90\% confidence limit on CSM interaction rate using the line-emission model.\label{tab:CSMRateBounds}}
\tablewidth{0pt}
\tabletypesize{\small}
\tablehead{
    \colhead{$S$} & \colhead{$t_\text{start}$ [days]} & \multicolumn2c{\galex [\%]} & \multicolumn2c{\hst [\%]} & \multicolumn2c{All UV [\%]} & \colhead{$r_\text{CSM}$\tablenotemark{a} [\SI{e16}{\centi\meter}]} & \colhead{$t_\text{erupt}$\tablenotemark{b} [yr]}
}
\decimals
\startdata
% scale factor      t_start     GALEX   HST     All     r_csm   t_erupt
90-100              & 0-500     & 0.65  & 11.   & 1.6   & 0-9   & 0-270     \\
(\sim\text{05gj})   & 500-1000  & 1.4   & 4.2   & 1.0   & 9-17  & 270-540   \\
                    & 1000-1500 & 7.6   & 13.   & 5.0   & 17-26 & 540-820   \\
                    & 1500-2000 & 21.   & 57.   & 17.   & 26-35 & 820-1100  \\
\hline
9-11                & 0-500     & 2.7   & 14.   & 5.1   & 0-9   & 0-270     \\
(\sim\text{11kx})   & 500-1000  & 6.2   & 4.7   & 2.7   & 9-17  & 270-540   \\
                    & 1000-1500 & 23.   & 13.   & 9.0   & 17-26 & 540-820   \\
                    & 1500-2000 & 57.   & 57.   & 36.   & 26-35 & 820-1100  \\
\hline
0.9-1.1             & 0-500     & 23.   & 18.   & 14.   & 0-9   & 0-270     \\
(\sim\text{15cp})   & 500-1000  & 31.   & 5.5   & 4.8   & 9-17  & 270-540   \\
                    & 1000-1500 & 77.   & 15.   & 13.   & 17-26 & 540-820   \\
                    & 1500-2000 & 77.   & 57.   & 44.   & 26-35 & 820-1100  \\
\hline
0.1-0.2             & 0-500     & 77.       & 17.   & 16.   & 0-9   & 0-270    \\
(\sim\text{18tb})   & 500-1000  & 77.       & 9.0   & 8.6   & 9-17  & 270-540   \\
                    & 1000-1500 & \nodata\tablenotemark{c}   & 21.   & 21.   & 17-26 & 540-820   \\
                    & 1500-2000 & \nodata   & 77.   & 77.   & 26-35 & 820-1100  \\
\enddata
\tablenotetext{a}{Corresponding radius of the innermost shell of CSM assuming an ejecta velocity $v_\text{ej}\approx\SI{20000}{\kilo\meter\per\second}$ \citep{Garavini2005-SN1999ac}.}
\tablenotetext{b}{Eruption time in years before the SN Ia explosion for material at $r_\text{CSM}$, assuming a shell expansion velocity $v_\text{exp}\approx\SI{100}{\kilo\meter\per\second}$ \citep{Dilday2012-PTF11kx}.}
\tablenotetext{c}{Indicates no \sneia were excluded by \galex observations in this range.}
\end{deluxetable*}

==> 2021 SNe Ia-CSM in GALEX 2021-11-18/nearby_historical.tex <==
\begin{deluxetable*}{llllll}
\tablecaption{Supernovae observed by GALEX only after discovery\label{tab:nearby-historical}}
\tablehead{
\colhead{Name} & \colhead{Date} & \colhead{NUV} &
\colhead{FUV} & \colhead{$t_{\rm first}$} & \colhead{$t_{\rm last}$} \\
\colhead{} & \colhead{(YYYY-MM-DD)} & \colhead{[\#]} & \colhead{[\#]} &
\colhead{[days]} & \colhead{[days]}
}
\startdata
SN1937D& 1937-09-09& 0&  1&25295&25295 \\
SN1954B& 1954-04-27& 3&  3&17952&19342 \\
SN1957A& 1957-02-26&14& 17&17128&19016 \\
SN1960F& 1960-04-17& 0&  4&17167&18278 \\
SN1960H& 1960-06-18& 2&  2&15984&16690 \\
\enddata
\tablecomments{Table~\ref{tab:nearby-historical} is published in its entirety in the electronic 
edition of the {\it Astrophysical Journal}.  A portion is shown here 
for guidance regarding its form and content.}
\end{deluxetable*}

==> 2021 SNe Ia-CSM in GALEX 2021-11-18/newz.tex <==
\begin{deluxetable}{ccccc}
\tablecaption{SNe Ia with updated redshifts derived in this work.
\label{tab:manualz}}
\tablehead{
    \colhead{Name} & \colhead{Catalog Redshift} & \colhead{New Redshift} & \colhead{Data Source} & \colhead{Measurement Type}
}
\startdata
SN~2009cp & 0.22 & $0.225\pm0.008$ & WISeREP & SNID \\
SN~2009cu & 0.10 & $0.099\pm0.003$ & WISeREP & SNID \\
SN~2009kt & 0.27 & $0.27592\pm0.00005$ & Gemini & host-galaxy lines \\
SN~2009kv & 0.32 & $0.315\pm0.008$ & Gemini & SNID \\
SN~2009kx & 0.23 & $0.217\pm0.003$ & Gemini & SNID \\
\enddata
\end{deluxetable}


==> 2021 SNe Ia-CSM in GALEX 2021-11-18/scale_factors.tex <==
\begin{deluxetable*}{lDDDl}
\tablecaption{\normalsize Scale factors for reference \snecsm from \Halpha line luminosity ratios.\label{tab:ReferenceScaleFactors}}
\tabletypesize{\small}
\tablewidth{0pt}
\tablehead{
    \colhead{SN} & \multicolumn2c{$L_{\text{H}\alpha}$} & \multicolumn2c{$S$} & \multicolumn2c{Epoch} & \colhead{Source}
    \vspace{-2pt} \\
    \colhead{} & \multicolumn2c{[$10^{39}$ erg/s]} & \multicolumn2c{} & \multicolumn2c{[days]} & \colhead{}
}
\decimals
\startdata
SN 2005gj   & 118.  & 54.   & +111 & \citet{Prieto2007-SN2005gj}     \\
PTF11kx     & 40.6  & 19.   & +371  & \citet{Silverman2013-PTF11kx}   \\
SN 2015cp   & 2.2   & 1     & +694  & \citet{Graham2019-SN2015cp}     \\
ASASSN-18tb/SN 2018fhw      & 0.22  & 0.10  & +139  & \citet{Kollmeier2019-SN2018fhw} \\
ATLAS18qtd/SN 2018cqj       & 0.038 & 0.02  & +193  & \citet{Prieto2020-SN2018cqj}    \\
\enddata
\end{deluxetable*}

==> 2021 SNe Ia-CSM in GALEX 2021-11-18/short_sample.tex <==
\movetabledown=2in
\begin{rotatetable*}
\newcolumntype{z}{>{\raggedright\arraybackslash}p{1.75in}}
\begin{deluxetable*}{lcllrRrrDr@{$\pm$}llz}
\tablecaption{\normalsize Basic information for our sample of \sneia.
\label{tab:Targets}}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tablehead{
\colhead{Target Name} & \colhead{Disc. Date} & \colhead{R.A.} & \colhead{Dec.} &  
\colhead{Obs.\tablenotemark{1}} & \colhead{$t_\text{first}$\tablenotemark{2}} & 
\colhead{$t_\text{last}$\tablenotemark{3}} & \colhead{$t_\text{next}$\tablenotemark{4}} & 
\multicolumn2c{Redshift} & \multicolumn2c{Distance} & \colhead{$A_V$\tablenotemark{5}} & \colhead{Reference(s)}
\vspace{-6pt} \\
\colhead{} & \colhead{} & \colhead{[h:m:s]} & \colhead{[d:m:s]} &
\colhead{} & \colhead{[days]} & 
\colhead{[days]} & \colhead{[days]} & 
\multicolumn2c{} & \multicolumn2c{[Mpc]} & \colhead{[mag]} & \colhead{}
}
\decimals
\startdata
ESSENCEg097 &  2004-10-05 &   $23:27:37.16$ &       $-09:35:21$ &            23 &           -407 &          2181 &           357 &    0.343 &       1464 &            103 &  0.086 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEg142 &  2004-10-09 &    $23:28:37.7$ &       $-08:45:04$ &            16 &            -35 &          2177 &           353 &    0.404 &       1725 &            121 &  0.078 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEg230 &  2004-10-17 &   $01:11:56.31$ &     $+00:07:27.7$ &            19 &           -376 &          2532 &          1081 &    0.392 &       1674 &            117 &  0.084 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEm027 &  2005-09-26 &   $01:09:15.01$ &     $+00:08:14.8$ &            14 &           -720 &          1870 &           742 &    0.289 &       1233 &             86 &  0.078 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEm043 &  2005-09-26 &   $23:29:51.73$ &     $-08:56:46.1$ &            16 &           -387 &          1825 &             1 &    0.266 &       1134 &             80 &  0.080 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEm062 &  2005-09-25 &  $01:09:52.902$ &    $+00:36:19.03$ &            14 &           -719 &          1829 &           729 &    0.314 &       1340 &             94 &  0.067 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEm075 &  2005-09-26 &   $23:24:42.29$ &     $-08:29:08.7$ &            16 &           -708 &          2209 &           360 &    0.102 &        423 &             30 &  0.099 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEn263 &  2005-11-22 &   $02:05:14.95$ &     $-04:56:39.1$ &            40 &           -410 &          1820 &          1421 &  0.36264 &       1549 &            109 &  0.070 &                                          \citet{2016SDSSD.C...0000:} \\
ESSENCEn278 &  2005-11-24 &   $23:28:17.55$ &     $-09:23:12.4$ &            22 &           -446 &          1766 &           296 &    0.304 &       1297 &             91 &  0.109 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEn326 &  2005-11-24 &   $23:29:58.59$ &     $-08:53:12.5$ &            16 &           -446 &          1766 &           291 &  0.26316 &       1128 &             79 &  0.082 &  \citet{2007SDSS6.C...0000:,2004SDSS3.C...0000:,2007ApJ...660..239K} \\
ESSENCEn400 &  2005-11-26 &   $01:13:13.26$ &     $-00:23:25.9$ &            16 &           -781 &          1767 &           676 &    0.424 &       1811 &            127 &  0.085 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEp425 &  2005-11-24 &   $23:29:56.19$ &     $-08:34:24.3$ &            20 &           -767 &          1766 &           291 &    0.458 &       1956 &            137 &  0.085 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEp434 &  2005-11-24 &   $01:12:40.25$ &     $+00:14:56.6$ &            15 &           -779 &          2129 &           683 &    0.339 &       1447 &            101 &  0.094 &                                          \citet{Miknaitis2007-ESSENCE} \\
ESSENCEq002 &  2006-09-16 &  $02:05:12.945$ &   $-03:39:00.723$ &            15 &          -1029 &          1546 &            64 &   0.3469 &       1482 &            104 &  0.064 &                                          \citet{narayan2016} \\
ESSENCEq022 &  2006-09-11 &  $01:12:03.864$ &  $-00:01:28.9452$ &            19 &          -1070 &          1838 &           387 &  0.22637 &        965 &             68 &  0.083 &                      \citet{2007SDSS6.C...0000:,2016SDSSD.C...0000:} \\
ESSENCEr185 &  2006-10-31 &  $01:11:48.245$ &    $-00:29:49.46$ &            12 &          -1120 &          1428 &           337 &  0.18011 &        767 &             54 &  0.066 &                      \citet{2007SDSS6.C...0000:,2016SDSSD.C...0000:} \\
ESSENCEr317 &  2006-11-14 &  $01:13:24.658$ &   $+00:51:27.757$ &            28 &           -778 &          1774 &           312 &   0.3361 &       1435 &            101 &  0.070 &                                          \citet{narayan2016} \\
Hawk        &  2004-11-05 &   $12:35:41.16$ &    $+62:11:37.19$ &           211 &           -281 &          2315 &           163 &  0.49673 &       2129 &            149 &  0.031 &                    \citet{2011AandA...528A..35M,2004AJ....127.3121W} \\
HST04Sas    &  2004-05-23 &  $12:36:54.125$ &    $+62:08:22.21$ &           213 &           -118 &          2481 &           329 &  0.44643 &       1914 &            134 &  0.031 &                      \citet{2004ApJ...617..240K,2004AJ....127.3121W} \\
\enddata
\tablenotetext{1}{Number of \galex observations in both bands}
\tablenotetext{2}{Number of days between the first \galex observation in either band and the discovery date}
\tablenotetext{3}{Number of days between the discovery date and the last \galex observation in either band}
\tablenotetext{4}{Number of days between the discovery date and the next \galex observation in either band}
\tablenotetext{5}{$V$-band galactic extinction}
% \tablenotetext{a}{Offset between NED entry and \galex sky coordinates is larger than 30 kpc}
\tablecomments{Table~\ref{tab:nearby-historical} is published in its entirety in the electronic 
edition of the {\it Astrophysical Journal}.  A portion is shown here 
for guidance regarding its form and content.}
\end{deluxetable*}
\end{rotatetable*}
